Three-Loop Evolution for Soft Functions of Exclusive $B$-Meson and Higgs Decays

We bootstrap the complete three-loop Lange--Neubert kernel for the leading-twist $B$-meson light-cone distribution amplitude in heavy quark effective theory by taking advantage of the conformal symmetry technique. In particular, we provide for the first time an all-order Wilson-line argument for the determination of the constant term in the LN kernel in terms of the light-quark, heavy-quark, and threshold soft anomalous dimensions. Remarkably, this innovative construction requires no additional three-loop diagrammatic calculations. Taking into account further the three-loop QCD evolutions for the hard and hard-collinear coefficient functions, the newly derived three-loop Lange--Neubert equation enables us to manifestly demonstrate the renormalization-group invariance of the soft-collinear factorization formula for the radiative leptonic $B_{u}^- \to \gamma \ell^{-} \bar \nu_{\ell}$ decay at leading power, validating our bootstrapped three-loop kernel and more importantly, our full bootstrap approach.

==> figures/diphoton-contour-symbol.tex <==
% Contour (c) as a cap with a right-facing foot.
\newcommand*{\diphotoncontour}{%
  \tikz[x=3.3pt,y=3.3pt,baseline=0pt]{%
    \draw[line width=.45pt,line join=round]
      (0,0)--(0,1.12)--(.9,1.12)--(.9,.22)--(1.51,.22);%
  }%
}

